Eradicating Attacks on the Internal Network with Internal Network Policy

In this paper we present three attacks on private internal networks behind a NAT and a corresponding new protection mechanism, Internal Network Policy, to mitigate a wide range of attacks that penetrate internal networks behind a NAT. In the attack scenario, a victim is tricked to visit the attacker's website, which contains a malicious script that lets the attacker access the victim's internal network in different ways, including opening a port in the NAT or sending a sophisticated request to local devices. The first attack utilizes DNS Rebinding in a particular way, while the other two demonstrate different methods of attacking the network, based on application security vulnerabilities. Following the attacks, we provide a new browser security policy, Internal Network Policy (INP), which protects against these types of vulnerabilities and attacks. This policy is implemented in the browser just like Same Origin Policy (SOP) and prevents malicious access to internal resources by external entities.

==> model.tex <==
\label{sec:model}
\subsection{Model}

In our model, there is an internal network, which one of its component is a device (probably a router) that acts as the network's default gateway. This device serves as NAT, protecting the network from external direct access to resources in the internal network (depicted in figure \ref{fig:homenetwork}).

\begin{figure}[h]
   \centering
   \begin{tabular}{@{}c@{\hspace{.5cm}}c@{}}
       \includegraphics[page=2,width=.45\textwidth]{INP.pdf}
   \end{tabular}
 \caption{Home network example}
 \label{fig:homenetwork}
\end{figure}

The goal of the adversary in our model is to gain access to the victim's internal network, only by making the victim browse to the adversary's controlled website.

\subsection{Assumptions}
A basic assumption is that the victim would surf to the attacker's website. We mention a couple of ways to achieve this:

\begin{itemize}
    \item {\bf Spear phishing \& social engineering} – the adversary can contact the victim by e-mail, social media or any other platform, and embed a link to its malicious website in a bate. Although there is more consciousness to information security, this method still works effectively \cite{phishing}.
    \item  {\bf 	Malicious third-party advertisement } - Many times, websites dynamically embed third-party resources, such as advertisements in iframes. So if an adversary can create an advertisement, which leads to its website, it can  appear in "innocent" websites on the internet, which the victim then visits.
\end{itemize}

\subsection{Technical Background}
\subsubsection{\textbf{SOP (Same Origin Policy)}}
Two URLs have the same origin if the protocol, port (if specified), and host are the same for both \cite{sop}. SOP is a critical security mechanism that restricts how a document or script loaded from one origin can interact with a resource from another origin. CORS (Cross-Origin Resource Sharing) \cite{cors}, is a mechanism which allows servers provide accessibility to resources, from different origins. CORS is based on HTTP headers which indicate what is the desired access to the resource. In special cases, where a complex HTTP request to a resource is initiated by a different origin resource, the browser triggers a preflight request, prior to the original one \cite{cors_preflight}. Only if the server responds with the relevant "allow" headers to the preflight request, the the original request is sent.
\subsubsection{\textbf{DNS Rebinding}} The concept was discovered more than two decades ago \cite{dean1996java}. In the attack flow, the victim is trying to resolve an attacker's controlled domain to an IP address. The attacker, which controls the response, answers with the first IP address, and sets the DNS TTL to a small value. Then, after a short period of time when the TTL is zero, the DNS record isn't cached anymore, and the victim tries to resolve again the attacker's domain. This time, the attacker responds with a second IP address, and the DNS Rebinding is completed. One of the main usages of rebinding attacks, is accessing devices in internal networks, while bypassing the SOP restrictions \cite{dns_rebinding_private_networks}.
\subsubsection{\textbf{The UPnP Protocol}}
UPnP stands for "Universal Plug and Play." Plug and Play describes devices that work with a computer system as soon as they are connected. Each network device, exposes its own UPnP API, according to the device functionality. For example, routers UPnP commands include adding port forwarding rules \cite{rfc6970}, setting the DNS server, querying network information etc. UPnP enabled devices, usually share in the LAN information about how connecting to their services, and which UPnP commands and API they support. This usually takes place with other protocols such as SSDP.


